Rankwidth meets stability

We study two notions of being well-structured for classes of graphs that are inspired by classic model theory. A class of graphs $C$ is monadically stable if it is impossible to define arbitrarily long linear orders in vertex-colored graphs from $C$ using a fixed first-order formula. Similarly, monadic dependence corresponds to the impossibility of defining all graphs in this way. Examples of monadically stable graph classes are nowhere dense classes, which provide a robust theory of sparsity. Examples of monadically dependent classes are classes of bounded rankwidth (or equivalently, bounded cliquewidth), which can be seen as a dense analog of classes of bounded treewidth. Thus, monadic stability and monadic dependence extend classical structural notions for graphs by viewing them in a wider, model-theoretical context. We explore this emerging theory by proving the following: - A class of graphs $C$ is a first-order transduction of a class with bounded treewidth if and only if $C$ has bounded rankwidth and a stable edge relation (i.e. graphs from $C$ exclude some half-graph as a semi-induced subgraph). - If a class of graphs $C$ is monadically dependent and not monadically stable, then $C$ has in fact an unstable edge relation. As a consequence, we show that classes with bounded rankwidth excluding some half-graph as a semi-induced subgraph are linearly $\chi$-bounded. Our proofs are effective and lead to polynomial time algorithms.

==> decoding.tex <==
\subsection{Decoding}\label{sec:decoding}
We now describe how the (suitably labeled) directed graph $\vec H$ encodes the original graph and how the adjacency relation of $G$ can be retrieved by means of a transduction.
The decoding (and thus the transduction) is defined in an inductive way. 

We now describe how we determine whether two vertices, $u,v\in U$ with respective colors $\chi(u)$ and $\chi(v)$ are adjacent in $G$.
We consider the parents $x=\pi(u)$ and $y=\pi(v)$ of $u$ and $v$ in $\widehat{T}$, the first level $\ell=1$ of the recursive tree and the vertex $\top(F)$ representing the factor $F=T$ at this level, and the colors $c_x=\chi(u)$ and  $c_y=\chi(v)$.

%The graph $G$ is encoded by the rooted tree $T$, with hierarchical partitions of the vertex set.
%To each level of the hierarchical partition corresponds a rooted forest, whose connected components correspond to the nodes of the higher level. At the highest level $p$ we have only a single node tree. At the leaves of the decompositions we have rooted trees whose leaves are the vertices of $G$.
At step $\ell$ of the induction process, we are given a factor $F\in\Upsilon$ at level $\ell$ (by means of $\top(F)$) with $u\wedge_T v\in F$,  $x=\pi_F(u)$, $y=\pi_F(v)$, $c_x=\chi_F(u)$,   and $c_y=\chi_F(v)$. 
The quotient tree $Y$ corresponding to the factorization of $F$ is determined from $\vec H$ and $\ell$.
Using the arcs defined in $\vec H$ we determine the factor $F_x$ of $x$ as well as the recoloring function corresponding to the path from $x$ to $\top(F_x)$ (put as a label on the arc from $x$ to $\top(F_x)$). From this we deduce $\gamma_x$, the representative color in the color class of $\kappa_F(u,\top(F_x))$ in the factorization. Similarly, we get $F_y$ and $\gamma_y$.

If $F_x=F_y$, i.e.\@ $x$ and $y$ are in the same factor, then we recurse in $F_x$, with the same $x,y,c_x,c_y$, but now at level $\ell+1$.
Otherwise, assume first that $Y$ is shallow with root $F_r$. If $F_x = F_r$, let $x' = x$ and $c_{x'} = c_x$; otherwise let
$x'$ be the parent in $T$ of $\top(F_x)$ and $c_{x'} = \rho(e_x)(\gamma_x)$ where $e_x$ is the edge linking $\top(F_x)$ to $x'$ in $T$. We define $y'$ and $c_{y'}$ analogously. It is easily checked that $x'=\pi_{F_r}(u)$, $c_{x'}=\chi_{F_r}(u)$, $y'=\pi_{F_r}(v)$, and $c_{y'}=\chi_{F_r}(v)$. We recurse in $F_r$ with $(x',y',c_{x'},c_{y'})$ at level $\ell+1$.

Otherwise, $Y$ is splendid. 
We consider the partition of $F$ driven by the pair of color classes $\gamma_x$, $\gamma_y$ (in fact, by the representatives of the color classes).
Using the arcs of $\vec H$ we logically define the top $\top(F_0)$ of the highest factor $F_0$ which is both the pruned top of a part $P_x$ (in the partitioning of $Y$) met by the leaf-to-root path from $x$ and the pruned top of a part $P_y$ met by the leaf-to-root path from $y$. 
Symmetrically, we consider the partition of $F$ driven by parts $\gamma_y$ and $\gamma_x$ and get the parts $P_x'$ and $P_y'$.
Note that the part $P_x$ cannot be a non-$\gamma_y$-subtree as $v\in U_{F_0}$ and, similarly, $P_y'$ cannot be a non-$\gamma_x$-subtree. Moreover, if $P_x$ is a mixed $(\gamma_x,\gamma_y)$-chain then $P_y'$ cannot be a mixed $(\gamma_y,\gamma_x)$-chain. Thus we can decide the adjacency of $u$ and $v$ as follows:

\begin{itemize}
	\item If $P_x\neq P_y$, then $F_0=F_x\wedge_Y F_y$, and we recurse in $F_0$, the computation of the new $x,y,c_x,c_y$ presenting no difficulties;
	\item If $P_x=P_y$ is a positive $(\gamma_x,\gamma_y)$-bloc we immediately deduce that $u$ and $v$ are adjacent;
	\item If $P_x=P_y$ is a negative  $(\gamma_x,\gamma_y)$-bloc we immediately deduce that $u$ and $v$ are non-adjacent.
	\item If $P_x=P_Y$ is a mixed $(\gamma_x,\gamma_y)$-chain, then we consider $P_x'$ and $P_y'$, instead. (And then we cannot have $P_x'=P_y'$ and $P_x'$ is a mixed $(\gamma_y,\gamma_x)$-chain.)
\end{itemize}


%	We first check whether we are in the case where the edge $e_y$ links the leaf containing $y$ to its parent $u$ and $u$ is in a mixed $(\gamma_x,\gamma_y)$-chain to which $x$ points to. If this is the case, then the $(\gamma_x,\gamma_y)$-type of $e_y$ gives the adjacency. (We similarly handle the symmetric case.) Otherwise we look at the greatest node $u$ so that  both $x$ and $y$ point to edges $e_x$ and $e_y$ linking $u$ to children of $u$. If one of the edges belong to a positive or negative bloc, we deduce the adjacency of $x$ and $y$. Otherwise $\mathsf{tp}_{\gamma_0}(e_x)$ and $\mathsf{tp}_{\gamma_0}(e_y)$ are both full and mixed, and we recurse in $T_u$ by considering $(x',\rho_{e_x}(c_x),y',\rho_{e_y}(y'))$, where $x'$ is the attachment vertex of $e_x$ in $T_u$ and $y'$ is the attachment vertex of $e_y$ in $T_u$.
%\end{enumerate}
